Ioco Theory for Probabilistic Automata

Model-based testing (MBT) is a well-known technology, which allows for automatic test case generation, execution and evaluation. To test non-functional properties, a number of test MBT frameworks have been developed to test systems with real-time, continuous behaviour, symbolic data and quantitative system aspects. Notably, a lot of these frameworks are based on Tretmans' classical input/output conformance (ioco) framework. However, a model-based test theory handling probabilistic behaviour does not exist yet. Probability plays a role in many different systems: unreliable communication channels, randomized algorithms and communication protocols, service level agreements pinning down up-time percentages, etc. Therefore, a probabilistic test theory is of great practical importance. We present the ingredients for a probabilistic variant of ioco and define the {\pi}oco relation, show that it conservatively extends ioco and define the concepts of test case, execution and evaluation.

==> eptcsdata.tex <==
\providecommand{\firstpage}{23}
\providecommand{\publicationstatus}{A.K. Petrenko, B.-H. Schlingloff, N. Pakulin (Eds.):\\
Tenth Workshop on Model-Based Testing (MBT 2015)\\
EPTCS 180, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.180.2}{10.4204/EPTCS.180.2}}
\pdfoutput=1

